ATSim3.5D: A Multiscale Thermal Simulator for 3.5D-IC Systems based on Nonlinear Multigrid Method

To resolve the rising temperatures in 3.5D-ICs, a thermal-aware design flow becomes increasingly crucial, necessitating an accurate and efficient thermal simulation tool. However, previous tools struggle to handle the unique heterogeneous multiscale structures in 3.5D-ICs and the nonlinear thermal effects caused by high temperatures. In this work, we present a multiscale thermal simulator for 3.5D-ICs. We propose a hybrid tree structure to generate multilevel grids and capture the multiscale features and employ the nonlinear multigrid method for quick solving. Compared to ANSYS Icepak, it exhibits high accuracy (mean absolute relative error <1%, max error $<\SI{2}{\degreeCelsius}$), and efficiency ($80\times$ acceleration), delivering a powerful means to evaluate and refine thermal designs.

==> color.tex <==
\definecolor{green1}{RGB}{0, 153, 0}
\definecolor{red1}{RGB}{255, 102, 0}
\definecolor{salmon}{RGB}{255,126,121}
\definecolor{orchid}{RGB}{122,129,255}
\definecolor{aqua}{RGB}{0,150,255}
\definecolor{tangerine}{RGB}{255,147,0}
\definecolor{maraschino}{RGB}{255,38,0}
\definecolor{clover}{RGB}{0,143,0}


==> doc/abstract.tex <==
\begin{abstract}
%This poses severe thermal challenges and calls for a thermal design flow, 
To resolve the rising temperatures in 3.5D-ICs, a thermal-aware design flow becomes increasingly crucial, necessitating an accurate and efficient thermal simulation tool. However, previous tools struggle to handle the unique heterogeneous multiscale structures in 3.5D-ICs and the nonlinear thermal effects caused by high temperatures.
In this work, we present a multiscale thermal simulator for 3.5D-ICs. 
We propose a hybrid tree structure to generate multilevel grids and capture the multiscale features and employ the nonlinear multigrid method for quick solving. 
Compared to ANSYS Icepak, it exhibits high accuracy (mean absolute relative error $<1\%$, max error $<\SI{2}{\degreeCelsius}$), and efficiency ($80\times$ acceleration), delivering a powerful means to evaluate and refine thermal designs.

\end{abstract}
